Let the Pretrained Language Models "Imagine" for Short Texts Topic Modeling

Topic models are one of the compelling methods for discovering latent semantics in a document collection. However, it assumes that a document has sufficient co-occurrence information to be effective. However, in short texts, co-occurrence information is minimal, which results in feature sparsity in document representation. Therefore, existing topic models (probabilistic or neural) mostly fail to mine patterns from them to generate coherent topics. In this paper, we take a new approach to short-text topic modeling to address the data-sparsity issue by extending short text into longer sequences using existing pre-trained language models (PLMs). Besides, we provide a simple solution extending a neural topic model to reduce the effect of noisy out-of-topics text generation from PLMs. We observe that our model can substantially improve the performance of short-text topic modeling. Extensive experiments on multiple real-world datasets under extreme data sparsity scenarios show that our models can generate high-quality topics outperforming state-of-the-art models.

==> tables/TQresult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!ht]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{LCSNTM}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multicolumn{16}{c}{StackOverflow}                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & 0.041  & 0.011          & -0.074         & -0.141         & 0.101          & 0.099          & 0.062      & 0.074      & -0.154                             & -0.183                             & -0.08       & -0.099     & -                    & -                    \\
                                     & RBO                                                                                & 0.985  & 0.989          & 0.814          & 0.925          & 0.995          & 0.979          & 0.927      & 0.92       & 0.790                              & 0.952                              & 0.99        & 0.992      & -                    & -                    \\ \midrule
\multirow{2}{*}{Extended Text (GPT2)} & NPMI                                                                               & 0.08   & 0.089          & 0.005          & -0.007         & 0.094          & 0.098          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.102}       & \textbf{0.115}       \\
                                     & RBO                                                                                & 0.99   & 0.992          & \textbf{0.998} & \textbf{0.996} & 0.996          & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.988                & 0.967                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text (T5)}   & NPMI                                                                               & 0.066  & 0.054          & 0.017          & 0.029          & 0.101          & \textbf{0.109} & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.109}       & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.998  & \textbf{0.997} & 0.997          & 0.996          & \textbf{0.999} & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.995                & 0.976                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.042  & 0.014          & -0.054         & -0.051         & 0.034          & 0.056          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.101}       & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.998  & \textbf{0.998} & 0.999          &                & \textbf{0.999} & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.995                & 0.978                \\ \midrule
\multicolumn{16}{c}{TagMyNews}                                                                                                                                                                                                                                                                                                                                                                       \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.040 & -0.062         & -0.063         & -0.086         & -0.009         & -0.006         & -0.032     & -0.029     & -0.134                             & -0.140                             & -0.059      & -0.057     & -                    & -                    \\
                                     & RBO                                                                                & 0.997  & 0.915          & 0.752          & 0.978          & 0.996          & 0.982          & 0.971      & 0.975      & 0.960                              & 0.986                              & 0.959       & 0.951      & -                    & -                    \\ \midrule
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.035  & 0.031          & 0.018          & \textbf{0.066} & \textbf{0.065} & 0.054          & -          & -          & -                                  & -                                  & -           & -          & 0.009                & 0.001                \\
                                     & RBO                                                                                & 0.951  & 0.981          & 0.999          & 0.998          & \textbf{0.999} & \textbf{0.994} & -          & -          & -                                  & -                                  & -           & -          & 0.985                & 0.971                \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & -0.001 & -0.012         & -0.022         & 0.016          & \textbf{0.034} & \textbf{0.039} & -          & -          & -                                  & -                                  & -           & -          & 0.007                & 0.012                \\
                                     & RBO                                                                                & 0.964  & 0.990          & \textbf{1.0}   & \textbf{0.997} & 0.999          & 0.994          & -          & -          & -                                  & -                                  & -           & -          & 0.993                & 0.978                \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.019  & 0.016          & 0.014          & 0.033          & \textbf{0.046} & \textbf{0.040} & -          & -          & -                                  & -                                  & -           & -          & 0.015                & 0.007                \\
                                     & RBO                                                                                & 0.983  & 0.993          & \textbf{1.0}   & \textbf{0.996} & 0.999          & 0.995          & -          & -          & -                                  & -                                  & -           & -          & 0.992                & 0.983                \\ \midrule
\multicolumn{16}{c}{WebSnippets}                                                                                                                                                                                                                                                                                                                                                                     \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.045 & -0.061         & -0.110         & -0.059         & 0.002          & 0.001          & 0.009      & 0.01       & -0.154                             & -0.136                             & -0.177      & -0.156     & -                    & -                    \\
                                     & RBO                                                                                & 0.994  & 0.997          & 0.999          & 0.759          & 0.999          & 0.998          & 0.918      & 0.953      & 0.944                              & 0.972                              & 0.996       & 0.992      & -                    & -                    \\ \midrule
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.013  & -0.024         & -0.048         & -0.058         & 0.020          & 0.008          & -          & -          & -                                  & -                                  & -           & -          & \textbf{0.028}       & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.998  & \textbf{0.999} & 0.999          & 0.997          & 0.999          & 0.996          & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.0}         & 0.978                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & 0.008  & -0.035         & -0.095         & -0.074         & \textbf{0.033} & 0.013          & -          & -          & -                                  & -                                  & -           & -          & 0.012                & \textbf{0.115}       \\
                                     & RBO                                                                                & 0.996  & 0.998          & \textbf{0.999} & 0.998          & \textbf{1.0}   & \textbf{0.999} & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.0}         & 0.967                \\ \cmidrule(l){2-16} 
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & -0.019 & -0.039         & -0.092         & -0.090         & \textbf{0.030} & 0.001          & -          & -          & -                                  & -                                  & -           & -          & 0.025                & \textbf{0.109}       \\
                                     & RBO                                                                                & 0.995  & 0.999          & \textbf{0.999} & 0.998          & \textbf{1.0}   & 0.997          & -          & -          & -                                  & -                                  & -           & -          & \textbf{1.0}         & 0.977                \\  \bottomrule 
\end{tabular}
}
\caption{Topic coherence (NPMI) and diversity (RBO) scores of topic words. $k$ is the topic number. The best in each case is shown in \textbf{bold}.}
\label{tab:topic_quality}
\end{table*}

==> tables/TQstackoverflow.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{Ours}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & 0.041       & 0.011     & -0.074      & -0.141      & 0.101      & 0.099      & 0.062      & 0.074      &                                    &                                    & -0.08      & -0.099      &                     &                     \\
                                     & RBO                                                                                & 0.985       & 0.989     & 0.814       & 0.925       & 0.995      & 0.979      & 0.927      & 0.92       &                                    &                                    & 0.99       & 0.992       &                     &                     \\
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.08        & 0.089     & 0.005       & -0.007      & 0.094      & 0.098      &            &            &                                    &                                    &            &             & 0.102               & 0.115               \\
                                     & RBO                                                                                & 0.99        & 0.992     & 0.998       & 0.996       & 0.996      & 0.994      &            &            &                                    &                                    &            &             & 0.988               & 0.967               \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & 0.066       & 0.054     & 0.017       & 0.029       & 0.101      & 0.109      &            &            &                                    &                                    &            &             & 0.109               & 0.109               \\
                                     & RBO                                                                                & 0.998       & 0.997     & 0.997       & 0.996       & 0.999      & 0.994      &            &            &                                    &                                    &            &             & 0.995               & 0.976               \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.042       & 0.014     & -0.054      & -0.051      & 0.034      & 0.056      &            &            &                                    &                                    &            &             & 0.101               & 0.109               \\
                                     & RBO                                                                                & 0.998       & 0.998     & 0.999       & 0.996       & 0.999      & 0.994      &            &            &                                    &                                    &            &             & 0.995               & 0.978               \\ \bottomrule 
\end{tabular}
}
\end{table*}

==> tables/TQtagmynews.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{Ours}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.040     & -0.062     & -0.063      & -0.086      & -0.009     & -0.006     & -0.032     & -0.029     &                                    &                                    & -0.059      & -0.057     &                      &                    \\
                                     & RBO                                                                                & 0.997      & 0.915      & 0.752       & 0.978       & 0.996      & 0.982      & 0.971      & 0.975      &                                    &                                    & 0.959       & 0.951      &                      &                    \\
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.035      & 0.031      & 0.018       & 0.066       & 0.065      & 0.054      &            &            &                                    &                                    &             &            & -0.009               & 0.115              \\
                                     & RBO                                                                                & 0.951      & 0.981      & 0.999       & 0.998       & 0.999      & 0.994      &            &            &                                    &                                    &             &            & 0.985                & 0.967              \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & -0.001     & -0.012     & -0.022      & 0.016       & 0.034      & 0.039      &            &            &                                    &                                    &             &            & -0.006               & 0.108              \\
                                     & RBO                                                                                & 0.964      & 0.990      & 1.0         & 0.997       & 0.999      & 0.994      &            &            &                                    &                                    &             &            & 0.993                & 0.976              \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & 0.019      & 0.016      & 0.014       & 0.033       & 0.046      & 0.040      &            &            &                                    &                                    &             &            & -0.193               & 0.109              \\
                                     & RBO                                                                                & 0.983      & 0.993      & 1.0         & 0.996       & 0.999      & 0.995      &            &            &                                    &                                    &             &            & 0.992                & 0.977              \\ \bottomrule 
\end{tabular}
}
\end{table*}

==> tables/TQwebsnippets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{3}{*}{Data}                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Topic\\ Quality\\ Metrics\end{tabular}} & \multicolumn{6}{c}{General Purpose Topic Models}                              & \multicolumn{6}{c}{Short Text Topic Models}                                                                                  & \multicolumn{2}{c}{\multirow{2}{*}{Ours}} \\ \cmidrule(lr){3-14}
                                     &                                                                                    & \multicolumn{2}{c}{LDA} & \multicolumn{2}{c}{CLNTM} & \multicolumn{2}{c}{CTM} & \multicolumn{2}{c}{BTM} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Graph\\ BTM\end{tabular}} & \multicolumn{2}{c}{NQTM} & \multicolumn{2}{c}{}                      \\ \cmidrule(l){3-16} 
                                     &                                                                                    & k=20        & k=50      & k=20        & k=50        & k=20       & k=50       & k=20       & k=50       & k=20                               & k=50                               & k=20       & k=50        & k=20                & k=50                \\ \midrule
\multirow{2}{*}{Short Text}          & NPMI                                                                               & -0.045     & -0.061     & -0.110      & -0.059      & 0.002      & 0.001      & 0.009      & 0.01       &                                    &                                    & -0.177      & -0.156     &                     &                     \\
                                     & RBO                                                                                & 0.994      & 0.997      & 0.999       & 0.759       & 0.999      & 0.998      & 0.918      & 0.953      &                                    &                                    & 0.996       & 0.992      &                     &                     \\
\multirow{2}{*}{Extended Text(GPT2)} & NPMI                                                                               & 0.013      & -0.024     & -0.048      & -0.058      & 0.020      & 0.008      &            &            &                                    &                                    &             &            & 0.028               & 0.109               \\
                                     & RBO                                                                                & 0.998      & 0.999      & 0.999       & 0.997       & 0.999      & 0.996      &            &            &                                    &                                    &             &            & 1.0                 & 0.978               \\
\multirow{2}{*}{Extended Text(T5)}   & NPMI                                                                               & 0.008      & -0.035     & -0.095      & -0.074      & 0.033      & 0.013      &            &            &                                    &                                    &             &            & 0.012               & 0.115               \\
                                     & RBO                                                                                & 0.996      & 0.998      & 0.999       & 0.998       & 1.0        & 0.999      &            &            &                                    &                                    &             &            & 1.0                 & 0.967               \\
\multirow{2}{*}{Extended Text(BART)} & NPMI                                                                               & -0.019     & -0.039     & -0.092      & -0.090      & 0.030      & 0.001      &            &            &                                    &                                    &             &            & 0.025               & 0.109               \\
                                     & RBO                                                                                & 0.995      & 0.999      & 0.999       & 0.998       & 1.0        & 0.997      &            &            &                                    &                                    &             &            & 0.999               & 0.977               \\ \bottomrule 
\end{tabular}
}
\end{table*}
